On the estimation of persistence intensity functions and linear representations of persistence diagrams

The prevailing statistical approach to analyzing persistence diagrams is concerned with filtering out topological noise. In this paper, we adopt a different viewpoint and aim at estimating the actual distribution of a random persistence diagram, which captures both topological signal and noise. To that effect, Chazel and Divol (2019) proved that, under general conditions, the expected value of a random persistence diagram is a measure admitting a Lebesgue density, called the persistence intensity function. In this paper, we are concerned with estimating the persistence intensity function and a novel, normalized version of it -- called the persistence density function. We present a class of kernel-based estimators based on an i.i.d. sample of persistence diagrams and derive estimation rates in the supremum norm. As a direct corollary, we obtain uniform consistency rates for estimating linear representations of persistence diagrams, including Betti numbers and persistence surfaces. Interestingly, the persistence density function delivers stronger statistical guarantees.

==> experiments.tex <==
\section{Experiments}
We apply our framework on the ORBIT5K data set, one that has been widely used in TDA literature \cite{adams2017persistence}. 

\begin{figure}\label{fig:ORBIT5K-orbits}
\centering
\begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/ORBIT5K/sample_orbit_r2.5.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/ORBIT5K/sample_orbit_r4.0.png}
     \end{subfigure}
        \caption{Sample orbits from the ORBIT5K data set with $r=2.5$ (left) and $r = 4.0$ (right)}
\end{figure}

\begin{figure}\label{fig:ORBIT5K-sample-diagram}
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering 
\includegraphics[width = \textwidth]{imgs/ORBIT5K/sample_diagram_r2.5.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering 
\includegraphics[width = \textwidth]{imgs/ORBIT5K/sample_diagram_r4.0.png}
\end{subfigure}
\caption{Sample persistent diagrams from the ORBIT5K data set}
\end{figure}

\begin{figure}\label{fig:ORBIT5K-KIE}
\centering 
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr2.5n1.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr4.0n1.png}
\end{subfigure}

\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr2.5n10.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr4.0n10.png}
\end{subfigure}

\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr2.5n100.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr4.0n100.png}
\end{subfigure}

\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr2.5n1000.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width = \textwidth]{imgs/ORBIT5K/KIEr4.0n1000.png}
\end{subfigure}
\caption{Kernel estimators for the persistence intensity function from the ORBIT5K data set with $r=2.5$ (left) and $r=4.0$ (right) and sample sizes $1,10,100,1000$ (top to bottom)}
\end{figure}
